20 Years of DDoS: a Call to Action

Botnet Distributed Denial of Service (DDoS) attacks are now 20 years old; what has changed in that time? Their disruptive presence, their volume, distribution across the globe, and the relative ease of launching them have all been trending in favor of attackers. Our increases in network capacity and our architectural design principles are making our online world richer, but are favoring attackers at least as much as Internet services. The DDoS mitigation techniques have been evolving but they are losing ground to the increasing sophistication and diversification of the attacks that have moved from the network to the application level, and we are operationally falling behind attackers. It is time to ask fundamental questions: are there core design issues in our network architecture that fundamentally enable DDoS attacks? How can our network infrastructure be enhanced to address the principles that enable the DDoS problem? How can we incentivize the development and deployment of the necessary changes? In this article, we want to sound an alarm and issue a call to action to the research community. We propose that basic research and principled analyses are badly needed, because the status quo does not paint a pretty picture for the future.

==> volumetric.tex <==
\section{DDoS Attacks}\label{sec:volumetric}

There is not one type of DDoS, there are a variety of TTPs.  Some are called ``low-and-slow'' (which starve servers of resources, and can be hard to detect), 
some are volumetric (which send overwhelming amounts of traffic that congest network links and overload servers, and which are hard to stop even though they are detectable by nature).
There is a large body of literature that broadly proposes DDoS taxonomies~\cite{mirkovic2004taxonomy,asosheh2008comprehensive,ddos-protection-center}.
In many cases, a large amount of effort has been focused on more than just DDoS attacks, themselves, but also include malcode ecosystem aspects (such as the toolchains 
used to compromise machines, etc.).
In many cases, prior DDoS descriptions include implementation details and malcode behavioral differences in efforts to enumerate the non-stationary space of 
malcode itself, the infection vectors, and the attack TTPs involved in DDoS attacks.
To highlight the status of our war on DDoS, here,
we focus primarily on the natures of DDoS attacks, and for clear illustration, we further focus briefly (below) on one specific common type: the clear-and-present threat posed by 
volumetric DDoS.\footnote{We note that
singling our volumetric attacks is not meant to undercut the importance of other types of DDoS or to suggest our observations are limited to them, but simply to present 
some specifics of one common type of attack.}

$\langle$ detection vs. remediation $\rangle$

{\bf What volumetric DDoS looks like, today}
Large volumes of DDoS attack traffic (sometimes called ``packet love''), result in very expensive infrastructure and deployments.
In considering what volumetric DDoS looks like, we observe that the largest recorded DDoSes have all been stateless and attacking sources in these attacks have capitalized on
their ability to spoof (or ``lie about'') the source addresses of their attack traffic 
(e.g. the 2016 Dyn and the 2016 krebsonline.com attacks~\cite{mansfield2016ddos, krebs2016krebsonsecurity}).
% TTPs of today’s volumetric DDoS attacks
% Spoofed vs. non-spoofed source-addresses
In short, the TTPs of the largest DDoS attacks seen today rely heavily on being able to spoof addresses (even if that is just to leverage an online service for an
amplification factor).
% Shift of usage from stateful to stateless transport protocol

$\langle$ Observe fundmantal weakness, long existance, growing ease of use, lack of fundmanetal remediation techniques: unmaintainable asymmetry $\dots \rangle$

While this is not a new typew of DDoS, the increasingly relative ease of acquiring the disruptive power of large volume attack sources has eleveated the appeal of stateless
DDoS attacks.
% Reflective amplification vs. direct
Whereas there continue to be attacks that leverage Secure Socket Layer (SSL) semantics, Transport Layer Security (TLS) semantics, or other sorts of stateful attack TTPs,
lately stateless attacks have shown to be the most destructive.
% Stateful (i.e. TCP-based, not just SYN-flood) attacks have become less common, and have not approached the scale of stateless attacks
Stateful attacks (i.e. those using active connections, and not simple SYN-floods) have become less of a threat when compared the prevalance, ease, and scale of stateless attacks.
% UDP (DNS, SNMP, NTP, etc.)
Key to this type of attack is the use of datagrams with spoofed source addresses.  These may be Domain Name System (DNS) queries, Simple Network Mangement Protocol (SNMP) queries,
Network Time Protocol (NTP) queries, {\tt memcached} queries, or others.
% Some are direct attacks from well provisioned sources
% SYN floods (with data) (MIRAI, XOR, etc.)
Some stateless attacks may also be spoofed control traffic for TCP connections.  For example, TCP SYN packets that have spoofed source addresses and large data payloads (even though SYN 
packets are not permitted to carry data on setup~\cite{postel1981rfc})~\cite{xor-attacks-csoonline}.



